Memory-constrained Vectorization and Scheduling of Dataflow Graphs for Hybrid CPU-GPU Platforms

The increasing use of heterogeneous embedded systems with multi-core CPUs and Graphics Processing Units (GPUs) presents important challenges in effectively exploiting pipeline, task and data-level parallelism to meet throughput requirements of digital signal processing (DSP) applications. Moreover, in the presence of system-level memory constraints, hand optimization of code to satisfy these requirements is inefficient and error-prone, and can therefore, greatly slow down development time or result in highly underutilized processing resources. In this paper, we present vectorization and scheduling methods to effectively exploit multiple forms of parallelism for throughput optimization on hybrid CPU-GPU platforms, while conforming to system-level memory constraints. The methods operate on synchronous dataflow representations, which are widely used in the design of embedded systems for signal and information processing. We show that our novel methods can significantly improve system throughput compared to previous vectorization and scheduling approaches under the same memory constraints. In addition, we present a practical case-study of applying our methods to significantly improve the throughput of an orthogonal frequency division multiplexing (OFDM) receiver system for wireless communications.

==> dxconfig/archmex <==
#!/usr/bin/env bash

################################################################################
# Archive a copy of the given file in a specified directory.
# The directory in which to place the archive is
# is specified by the setting of the \verb#lxdir# variable in the script.
#
# Side effect: this script sets the directory navigation label
# \verb#archmez#. Any previous setting for this label is lost.
# Upon exit, the label points to the directory corresponding to 
# the value of \verb#lxdir#.
#
# Configuration variable: old (change this to select a new subdirectory or
# path in which to store the archived file copies)
################################################################################

lxprog=archmex

# Configuration variable:
lxdir="/Users/ssb/Dropbox/tmp/bkp-2017/sep-2017"

if [ $# -ne 1 ]; then
    echo $lxprog error: arg count
    exit 1
fi

lxarg="$1"
dxpushd .
cd "$lxdir"

if [ $? -ne 0 ]; then
    echo $lxprog error: could not find subdirectory \"$lxdir\"
    dxpopd
    exit 1
fi

dlk archmez
cd ..
dxpopd

sutsvcp archmez "$lxarg"
if [ $? -ne 0 ]; then
    echo $lxprog error: problem saving file
    exit 1
fi



==> dxconfig/showme <==
#!/usr/bin/env bash

# Retrieve a copy of a previous revision of a file, given the 
# commit number and name of the file,

# Usage: showme <commit ID> <filename>

lxprog=showme

lxpath=papers/SIPS2016
lxdir=showme-results

if [ $# -ne 2 ]; then
    echo $lxprog error: arg count
    exit 1
fi

if ! [ -d "$lxdir" ]; then
    echo $lxprog error: cannot find directory \"$lxdir\"
    exit 1
fi

lxcommit="$1"
lxfile="$2" 

git show "$lxcommit":"$lxpath"/"$lxfile" > "$lxdir"/"$lxfile"


